Fast simulation of bosonic qubits via Gaussian functions in phase space

Bosonic qubits are a promising route to building fault-tolerant quantum computers on a variety of physical platforms. Studying the performance of bosonic qubits under realistic gates and measurements is challenging with existing analytical and numerical tools. We present a novel formalism for simulating classes of states that can be represented as linear combinations of Gaussian functions in phase space. This formalism allows us to analyze and simulate a wide class of non-Gaussian states, transformations and measurements. We demonstrate how useful classes of bosonic qubits -- Gottesman-Kitaev-Preskill (GKP), cat, and Fock states -- can be simulated using this formalism, opening the door to investigating the behaviour of bosonic qubits under Gaussian channels and measurements, non-Gaussian transformations such as those achieved via gate teleportation, and important non-Gaussian measurements such as threshold and photon-number detection. Our formalism enables simulating these situations with levels of accuracy that are not feasible with existing methods. Finally, we use a method informed by our formalism to simulate circuits critical to the study of fault-tolerant quantum computing with bosonic qubits but beyond the reach of existing techniques. Specifically, we examine how finite-energy GKP states transform under realistic qubit phase gates; interface with a CV cluster state; and transform under non-Clifford T gate teleportation using magic states. We implement our simulation method as a part of the open-source Strawberry Fields Python library.

==> infidelities.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
log basis x={10},
log basis y={10},
tick align=outside,
tick pos=both,
x grid style={white!69.0196078431373!black},
xlabel={Squeezing parameter \(\displaystyle r\)},
xmin=0.0082234015942689, xmax=0.608020895329329,
xmode=log,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Infidelity \(\displaystyle 1-F\)},
ymin=6.34470001922197e-05, ymax=1.42921444808959,
ymode=log,
ytick style={color=black}
]
\addplot [semithick, color0, mark=+, mark size=3, mark options={solid}, only marks]
table {%
0.01 0.000100059993590196
0.01144419297975 0.000131029543874228
0.0130969552957759 0.000171590223381313
0.0149884083852018 0.000224712365105351
0.0171530238019552 0.000294286196228843
0.019630251457582 0.000385406732133164
0.0224652385921587 0.00050474689045088
0.0257096525784791 0.000661046162418577
0.0294226225550442 0.000865750620128503
0.033671817049027 0.00113385113354181
0.0385346772287901 0.00148498117720652
0.0440998282618652 0.00194485462577199
0.0504686945002617 0.00254714882566465
0.0577573479297042 0.00333597084685333
0.0660986235706098 0.00436908752188647
0.0756445403837911 0.00572215581307556
0.0865690718016596 0.00749426330590974
0.0990713163776025 0.00981518456831121
0.113379126338315 0.0128548847720926
0.129753260169113 0.0168359665434619
0.148492134912704 0.022049971547779
0.169937264791605 0.0288787306023502
0.1944794852726 0.0378223258241992
0.222566076006208 0.0495357125305176
0.254708912456075 0.0648766827789414
0.291493794780957 0.0849686830031443
0.333591123987291 0.111283085991199
0.381768119924226 0.145746942130131
0.436902803792918 0.190884100731671
0.5 0.250000036003604
};
\addlegendentry{$n=$1}
\addplot [semithick, color1, mark=x, mark size=3, mark options={solid}, only marks]
table {%
0.01 0.000300043927307758
0.01144419297975 0.000392935944229955
0.0130969552957759 0.000514594049462969
0.0149884083852018 0.000673914443108492
0.0171530238019552 0.000882565512136946
0.019630251457582 0.00115580340610455
0.0224652385921587 0.00151361127575378
0.0257096525784791 0.0019821446947117
0.0294226225550442 0.00259563303927324
0.033671817049027 0.00339886241030718
0.0385346772287901 0.004450413527187
0.0440998282618652 0.00582687942203619
0.0504686945002617 0.00762835115087357
0.0577573479297042 0.00998553593625517
0.0660986235706098 0.0130689657538773
0.0756445403837911 0.0171008626726075
0.0865690718016596 0.0223703437504739
0.0990713163776025 0.0292527603739438
0.113379126338315 0.0382340413006361
0.129753260169113 0.0499408841807655
0.148492134912704 0.0651773975330835
0.169937264791605 0.084968116726854
0.1944794852726 0.110605810138378
0.222566076006208 0.143699456246932
0.254708912456075 0.186211976581797
0.291493794780957 0.240466596110556
0.333591123987291 0.309081315430707
0.381768119924226 0.394756400517455
0.436902803792918 0.499778749432252
0.5 0.625000012001202
};
\addlegendentry{$n=$2}
\addplot [semithick, color2, mark=*, mark size=3, mark options={solid}, only marks]
table {%
0.01 0.000572948037478316
0.01144419297975 0.000818277858882221
0.0130969552957759 0.00101652946868325
0.0149884083852018 0.00134710552313067
0.0171530238019552 0.00176570082163408
0.019630251457582 0.00230890559930419
0.0224652385921587 0.00302556358127493
0.0257096525784791 0.00396117406411922
0.0294226225550442 0.00518586898356732
0.033671817049027 0.00678874057028178
0.0385346772287901 0.00888535862411444
0.0440998282618652 0.01162727118833
0.0504686945002617 0.0152113248894785
0.0577573479297042 0.0198933346746066
0.0660986235706098 0.0260047536545049
0.0756445403837911 0.0339735926354291
0.0865690718016596 0.0443500114064357
0.0990713163776025 0.0578367774531732
0.113379126338315 0.0753240423074515
0.129753260169113 0.0979262068082628
0.148492134912704 0.127015668819957
0.169937264791605 0.16424283532408
0.1944794852726 0.211522527887271
0.222566076006208 0.270951684466609
0.254708912456075 0.34459944494351
0.291493794780957 0.434076134438579
0.333591123987291 0.539743901038718
0.381768119924226 0.659393526685517
0.436902803792918 0.786231536156825
0.5 0.906250001714458
};
\addlegendentry{$n=$3}
\end{axis}

\end{tikzpicture}

